When to Trust Your Data: Enhancing Dyna-Style Model-Based Reinforcement Learning With Data Filter

Reinforcement learning (RL) algorithms can be divided into two classes: model-free algorithms, which are sample-inefficient, and model-based algorithms, which suffer from model bias. Dyna-style algorithms combine these two approaches by using simulated data from an estimated environmental model to accelerate model-free training. However, their efficiency is compromised when the estimated model is inaccurate. Previous works address this issue by using model ensembles or pretraining the estimated model with data collected from the real environment, increasing computational and sample complexity. To tackle this issue, we introduce an out-of-distribution (OOD) data filter that removes simulated data from the estimated model that significantly diverges from data collected in the real environment. We show theoretically that this technique enhances the quality of simulated data. With the help of the OOD data filter, the data simulated from the estimated model better mimics the data collected by interacting with the real model. This improvement is evident in the critic updates compared to using the simulated data without the OOD data filter. Our experiment integrates the data filter into the model-based policy optimization (MBPO) algorithm. The results demonstrate that our method requires fewer interactions with the real environment to achieve a higher level of optimality than MBPO, even without a model ensemble.

==> 3_theory.tex <==
\section{Out-of-distribution data filter}


In Dyna-style algorithms, data points on \( \dreal \) are generated by \( \policy \) and \( \pp^* \). To enhance the performance of Dyna-style algorithms, a way is to filter out data points in \( \dest \) that are not likely to be generated by \( \policy \) and \( \pp^* \). Based on these intuitions, we introduce our Out of Distribution Data Filter in Algorithm~\ref{algo:DataFilter}. \sh{Make it clear how the data filter enters Algorithm~\ref{algo:modelbasedaddmodelfree}.}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/OODDataFilter.drawio.pdf}
    \caption{Visualization of out-of-distribution data filter.}
    \label{fig:OOD data filter}
\end{figure}


Line~\ref{algo:rej_rule} is the \ac{ood} rule, where we detect and discard all  those states in \( \dest \) that are far away from any state in \( \dreal \) as shown in Fig.~\ref{fig:OOD data filter}. The norm used in Line~\ref{algo:rej_rule} is the \( L_2 \) norm. The term \( \epsilon_k \) is the threshold of the distance between the current state and the closest state in \( \dreal \). We call \( \epsilon_k \) the \emph{reject level}.


Note that Line~\ref{algo:rej_rule} never eliminates the first-step data points from \(\dest\), regardless of how small the reject level \(\epsilon_k\) is, if we use branched rollouts as in \citet{janner_when_2019}. This is because, in branched rollouts, the initial states are picked from \(\dreal\), which means the closest state in \(dreal\) is itself. We will discuss the choice of \(\epsilon_k\) in Section~\ref{sec:exp}.

Additionally, Algorithm~\ref{algo:DataFilter} differs from an early stop strategy. As shown in Fig.~\ref{fig:OOD data filter}, for a simulated trajectory (depicted by the blue line), we do not filter out the last points; instead, we filter out the middle points. \yl{Please revise this sentence} \yw{TODO}
 

\begin{algorithm}
    \caption{\textsc{OOD-DataFilter}}
    \label{algo:DataFilter}
    \begin{algorithmic}[1]
        \Require \( \dreal \), \( \dest \), Episode number \( k \), Reject level \( \epsilon_k \)
        \Ensure \( \dreduct \)
        \State \( \dreduct \gets \dest \)
        \For{\( (s,a,s') \in \dest \)}
        \If{ \(\forall (s^*, \cdot, \cdot) \in \dreal\), such that \(\|s - s^*\| \geq \epsilon_k \) } \label{algo:rej_rule}
        \State eliminate \((s,a,s') \) from \(\dreduct\)
        \EndIf
        \EndFor
        \State \Return \( \dreduct \)
    \end{algorithmic}
\end{algorithm}


To show the reason why Algorithm~\ref{algo:DataFilter} leads to a better acceleration, we will show two results in the following subsections: 

\begin{enumerate}
    \item \emph{Bounding the data shifting}: Closer initial states leads to a lesser shifting in trajectories simulated by estimated model (Theorem~\ref{theorem: next_state_bound}).
    \item \emph{Bounding the value function update shifting}: Lesser shifting data points in \(\dreal\) leads to a closer update in \( Q \)-network (updated by data in \( \dest \)) to \( Q \)-network (updated by data points in \( \dreal \)) (Theorem~\ref{theorem: bound on excess error of value function}). \sh{The meaning of the statement is not clear to me. Your statements should still be understandable when all the contents in the parentheses are removed.}
\end{enumerate}

With the above two results, we can conclude that the filtered data set \( \dreduct \) leads to a better acceleration compared to \( \dest \). Thus, with Algorithm~\ref{algo:DataFilter}, the efficiency of Dyna-style algorithms is improved. In the next two subsections, we will formally state and prove these two results.

\subsection{Bounding the data shifting}

Fix episode \( k \), denote \( s \) as the state in a data point taken from \( \dreal \) and \( \hs \) as the state in a data point taken from \( \dest \). Consider an exploration strategy \( \pi_\phi \) parameterized by \( \phi \). The next state interacted with the real model is \( s' \sim \pp(s, \pi_\phi(s)) =\mathcal{N} (\mu(s, \pi_\phi(s)), \sigma^2(s, \pi_\phi(s)) )\) and the next state simulated from the estimated model is \( \hs' \sim \hpp(\hs, \pi_\phi(\hs)) = \mathcal{N} (\hat{\mu}(\hs, \pi_\phi(\hs)), \hat{\sigma}^2(\hs, \pi_\phi(\hs)) ) \).



%
\begin{assumption}\label{ass:trans_lips}
    The mean of the estimated transition kernel is Lipschitz, i.e.,
    \begin{equation}
        \|
        \muhat (s,a) - \muhat (\hs, a)
        \|
        \leq
        L_S \| \hs - s \|
    \end{equation}
    and
    \begin{equation}
        \|
        \muhat (s,a) - \muhat (s, \hat{a})
        \|
        \leq
        L_A \| \hat{a} - a \|
    \end{equation}
    for all \((s,a) \in S \times A \) and \((\hat{s},\hat{a}) \in S \times A \).
\end{assumption}
%
Assumption~\ref{ass:trans_lips} can be satisfied by adding a regularization term in the update of model neural network, See~\citet{zheng_is_2022} for example.
%
In addition, we assume that the policy network is Lipschitz. To simplify the analysis, we use \ac{DQN} \citep{mnih_human-level_2015} as the model-free algorithm instead of \ac{sac}, thus considering only a finite action space in this and the next subsection. For a finite action space, each \(\pi_{\phi}(s)\) can be viewed as a vector in \(\mathbb{R}^{|A|}\), and the norm on the policy is defined as the \(L_2\) norm. We now state the following assumption:

\begin{assumption}\label{ass:policy_lips}
    The policy \( \policy \) is Lipschitz, i.e.,
    \begin{equation}
        \| \pi_{\phi} (s) - \pi_{\phi}(\hs) \|
        \leq
        L_\phi \| \hs - s \|.
    \end{equation}
\end{assumption}

\sh{I suspect that there is a fundamental flaw in the main results. If I understand it correctly, $\dreal$ keeps data from different episodes. However, the policy is also updated after each episode. As a result, for a state-action pair $(s,a)$ recorded from an earlier episode, because the policy may have changed, the action given by the current policy is not necessarily close to $a$. Therefore, only checking the similarity based on $s$ is insufficient, even when $\policy$ is Lipschitz. (In fact, the statement in the assumption is ambiguous. Did you mean that $\pi_{\phi_h}^k$ is Lipschitz continuous for all $h$ and all $k$?}\yl{We actually tested the filter that includes actions, it performs badly. Maybe we should mention here that the policy do not change rapidly through episode and refer to papers such as TRPO?}\sh{You should do whatever needed to make your theory consistent. The technical results are suspicious given that $\policy$ is used (e.g., in Theorem~\ref{theorem: next_state_bound} and its proof) instead of $\pi_{\phi_h}^k$.}\yl{I get it, let us fix it by tomorrow.}

In order to measure the model estimation error, we introduce the following definition:
\begin{definition}[Kernel density estimation (KDE) and efficient sample size]
    We use a kernel function \(K_h\) with
    bandwidth \(h\) to estimate \(\mu (s, a)\) and \(\sigma (s, a)\):

    \[ \hat{\mu} (s, a) = \frac{\sum_{i = 1}^N K_h ((s, a) - (s_i, a_i))
            s_i'}{\sum_{i = 1}^N K_h ((s, a) - (s_i, a_i))},\]

    \begin{equation}
        \hat{\sigma}^2 (s,
        a) = \frac{\sum_{i = 1}^N K_h ((s, a) - (s_i, a_i)) (s_i' - \hat{\mu} (s,
            a))^2}{\sum_{i = 1}^N K_h ((s, a) - (s_i, a_i))} .
    \end{equation}

    The next state \(s_i'\) in sample \(i\) is drawn from \(s_i' \sim \mathbb{P}
    (s_i, a_i) =\mathcal{N} (\mu (s_i, a_i), \sigma^2 (s_i, a_i))\).
    The effective sample size \(n_{\mathrm{eff}}
    (s, a)\) is defined as:

    \[ n_{\mathrm{eff}} (s, a) = \sum_{i = 1}^N K_h ((s, a) - (s_i, a_i)) . \]
\end{definition}
If we choose kernel function \( K_h \) as index function, i.e., \( K_h(x) = 1 \) if \(x = 0\) and \(0\) elsewise. The KDE estimation reduces to the maximum likelihood estimation with \( n_{\mathrm{eff}} \) being the number of visitations.

\begin{theorem}\label{theorem: next_state_bound}
    Under assumption  \ref{ass:trans_lips} and \ref{ass:policy_lips}, given data point \((s, \cdot, \cdot) \in \mathcal{D}_{\mathrm{real}}\) and \((\hs, \cdot, \cdot) \in \mathcal{D}_{\mathrm{est}}\), with probability \((1 - \epsilon)(1- \epsilon_{\mathrm{KDE}})\) we have
    \begin{align}
        \| \hat{s}' (\hat{s}, \pi_{\phi} (\hat{s})) - s' (s, \pi_{\phi} (s)) \|
         & \leq
        (L_S + L_A L_\phi) \| \hs - s \|                                                                     \\
         & \quad +
        \sqrt{\frac{\sigma_{\pi_{\phi}(s)}^2 (s)}{n_{\mathrm{eff}} (s, \policy(s)) \epsilon_{\mathrm{KDE}}}} \\
         & \quad +
        \sqrt{\frac{\sigma^2_{\pi_{\phi} (\hat{s})} (\hat{s}) +
        \hat{\sigma}^2_{\pi_{\phi} (s)} (s)}{\epsilon}},
    \end{align}
    where \(\hat{s}' (\hat{s}, \pi_{\phi} (\hat{s})) \sim \hat{\mathbb{P}}
    (\hat{s}, \pi_{\phi} (\hat{s}))\) and \(s' (s, \pi_{\phi} (s)) \sim \mathbb{P}
    (s, \pi_{\phi} (s))\).
\end{theorem}

\begin{proof}
    See Appendix~\ref{pf:next_state_bound}.
\end{proof}

For deterministic transition, the bound can be simplified into:
\begin{corollary}\label{coro: next_state_deterministic}
    When the real transition \(\hp \) and estimated transition \(\hpp\) are both deterministic, the upper bound in theorem~\ref{theorem: next_state_bound} becomes:
    \begin{align}
        \| \hat{s}' (\hat{s}, \pi_{\phi} (\hat{s})) - s' (s, \pi_{\phi} (s)) \|
         & \leq
        (L_S + L_A L_\phi) \| \hs - s \|.
    \end{align}
\end{corollary}

% The estimated model can be regarded as an estimator of the real environment. The excess error, which contains estimation and approximation errors, is inevitable since the estimated model is trained with finite samples (even with fewer samples at an early stage) and within finite function space. The excess error would propagate to value function and policy through training.
%
Theorem~\ref{theorem: next_state_bound} bounds the shifting distance when simulate data from \( \hp \) under \( \policy \) if the distance between initial states is bounded. 
In the remaining analysis, we will show that the distance between the updated parameter of \( Q \)-network using data points from \( \dest \) and \( \dreal \) is bounded by the distance between data points shifting.

\subsection{Bounding the value function update shifting}
%
To formally state the theorem, we denote one data point from \( \dreal \) as \(d\triangleq[s,a,s']^{T}\) and one data point from \( \dest \) as \(\hat{d}\triangleq[\hat{s},\hat{a},\hat{s}^{'}]^{T}\).
We define the \( Q \)-network as \(Q (s, a ; \theta)\), where \(\theta\) represents the parameters.
%
The target value \(y\) is defined as
\begin{equation}
    y (s, a) = r (s, a) + \gamma \max_{a'} Q  (s', a' ; \theta^-),
\end{equation}
where \(s'\) is the next state, \(\theta^-\) are the parameters of the target network, which are periodically updated to match the \( Q \)-network parameters \(\theta\).
%
The Loss function \(L(\theta)\) of \ac{DQN} is defined as
%
\begin{equation}
    L (\theta) = \frac{1}{2} (y (s, a) - Q (s, a; \theta))^2.
\end{equation}
%
The update rule for the parameters of \( Q \)-network is
\begin{equation}
    \theta_{t + 1} \leftarrow \theta_t - \alpha \nabla_{\theta} L (\theta_t).
\end{equation}
%
By simple derivation, the above update rule becomes:
%
\begin{equation}
    \theta_{t + 1} \leftarrow \theta_t + \alpha (y (s, a) - Q (s, a ; \theta_t))
    \nabla_{\theta} Q (s, a ; \theta_t)
\end{equation}
%
The corresponding target and updates using a data point \((\hat{s} , \hat{a} , \hat{s} ')\) from \( \dest \) are:
%
\begin{equation}
    \hat{y} (\hat{s} , \hat{a} ) = r (\hat{s} , \hat{a} ) + \gamma \max_{a_1'} Q
    (\hat{s} ', \hat{a} ' ; \theta^-),
\end{equation}
%
and
%
\begin{equation}
    \hat{\theta}_{t + 1} \leftarrow \theta_t + \alpha (\hat{y} (\hat{s} ,
    \hat{a} ) - Q (\hat{s} , \hat{a}  ; \theta_t)) \nabla_{\theta} Q (\hat{s} ,
    \hat{a}  ; \theta_t).
\end{equation}
Before we proceed, we make the following assumptions on the \( Q \)-network and reward function:
%
%
\begin{assumption}\label{ass: lipschiz for Q}
    The reward function, gradient function of value function and value function itself are Lipschitz, i.e.,
    \begin{align}
        \|r(s,a)-r(\hs,\hat{a})\|                                                                              & \leq L_1\|d-\hat{d}\|, \\
        \|\nabla_{\theta} Q(s,a;\theta)-\nabla_{\theta} Q(\hs,\hat{a};\theta))\| & \leq L_2\|d-\hat{d}\|, \\
        \|Q(s,a;\theta)-Q(\hs,\hat{a};\theta))\|\,                                             & \leq L_3\|d-\hat{d}\|,
    \end{align}
    for all \( d \in S \times A \times S\) and \( \hat{d} \in S \times A \times S\). \sh{Relate $d$ to $(s,a)$.}
    In addition, the $\max_{a} Q  (s, a ; \theta^-)$ is also Lipschitz with respect to $s$, i.e.,
    \begin{align}
        \|\max_{a } Q  (s, a ; \theta^-)-\max_{a } Q  (\hs, a ; \theta^-)\|\leq L_4\|s-\hs\|.
    \end{align}
\end{assumption}
%
Furthermore, we assume those functions are finite.
\begin{assumption}\label{ass: varialbes bounded}
    There are existing finite constants $D_1\ge0$, $D_2 \ge 0$ and $D_3 \ge 0$, such that, $\|r( \cdot, \cdot )\|\leq D_1$, $\|\nabla_{\theta}Q( \cdot, \cdot ; \theta )\|\leq D_2$ and $\|Q( \cdot, \cdot ; \theta )\|\leq D_3$.
\end{assumption}
%
\sh{Discuss any assumptions made. At this point, reviewers may start to question whether some of the assumptions hold in practice.}
Now, we state the thereorem:
\begin{theorem}\label{theorem: bound on excess error of value function}
    Under assumption~\ref{ass: lipschiz for Q} and~\ref{ass: varialbes bounded}, for any \(\gamma>0\) and \(\alpha>0\), it holds for any \(\theta^{-}\), \((s,a,s')\) and \((\hat{s} , \hat{a} , \hat{s} ')\):
    \begin{align}
        \| \hat{\theta}_{t + 1} - \theta_{t + 1} \| & \leq C_1(\alpha, \gamma) \| d - \hat{d} \|^2+C_2(\alpha,\gamma)\| d - \hat{d}  \|
    \end{align}
    where
    \begin{align}
        C_1(\alpha, \gamma) & =\alpha  (L_1 L_2 + L_3 L_2+\gamma L_4 L_2)                   \\
        C_2(\alpha,\gamma)  & =\alpha   L_2 D_2                                             \\
                            & \quad+ \alpha\left( \gamma L_1 + L_3 + \gamma L_4 \right) D_1 \\
                            & \quad+ \alpha(1+\gamma) L_2 D_3.
    \end{align}
\end{theorem}
\begin{proof}
    The proof is attached in Appendix~\ref{proof: bound on excess error of value function}.
\end{proof}

Now, if the policy \( \policy \) is deterministic, we can denote \(d=[s,\pi_{\phi}(s),s' (s, \pi_{\phi} (s))]^{\top}\) and \(\hat{d}=[\hat{s},\pi_{\phi}(\hat{s}),\hat{s}' (\hat{s}, \pi_{\phi} (\hat{s}))]^{\top}\). If both \( \hp \) and \( \pp^{\ast} \) are deterministic. By Assumption~\ref{ass:policy_lips} and Corollary~\ref{coro: next_state_deterministic}, we have
%
\begin{equation}
    \|d-\hat{d}\|\leq C_{3}\|s-\hs\|,
\end{equation}
%
where \(C_3 \triangleq \left(1+L_S+L_{\phi}+L_{A}L_{\phi}\right)\). Then, we have the following corollary:
%
\begin{corollary}
    Under Assumption~\ref{ass:policy_lips}, with Corollary~\ref{coro: next_state_deterministic} and a deterministic policy \( \policy \), the upper bound in theorem~\ref{theorem: bound on excess error of value function} becomes
    \begin{align}
        \| \hat{\theta}_{t + 1} - \theta_{t + 1} \| & \leq C_1(\alpha, \gamma)C_{3}^{2}\|s-\hs\|^{2} \\
                                                    & \quad+C_2(\alpha, \gamma)C_3\|s-\hs\|.
    \end{align}
\end{corollary}
%
%
% Theorem~\ref{theorem: bound on excess error of value function} states that the update  of \( Q \)-network's parameters using \( \hat{d} \) from \( \dest \) is close to \( \theta_{t + 1} \) using \( d \) from \( \dreal \).  Combining with Theorem~\ref{theorem: next_state_bound}, if we can bound the distance between \( s \) and \( \hs \), then we can bound the updated parameters updated by data points from \( \dreal \) and \( \dest \).

One implication of Theorem~\ref{theorem: next_state_bound} is that data simulated from the estimated model closely approximates data interacted from the real model when given a similar initial state. As a result of that, together with Corollary~\ref{coro: next_state_deterministic}, a similar initial state makes the \( Q \)-network's updated parameters \( \hat{\theta}_{t + 1} \) updated using data simulated from estimated model close to the updated parameters \( \theta_{t + 1} \) updated using data interacted with real environment. This increases the reliability and efficiency of the model-free training process. The analysis of this section provides a reason why Algorithm~\ref{algo:DataFilter} can enhance the performance of Dyna-style algorithms. In the next section, we will show empirically that the  \ac{mbpo} with out-of-distribution data filter using a single model network outperforms \ac{mbpo} with an ensemble of model networks.


% The goal of Algorithm~\ref{algo:DataFilter} is to filter out data that deviates significantly from data interacted from the real model. The filtering rule is specified in Line~\ref{algo:rej_rule}. The term \( \epsilon_k \) represents the confidence interval maintained in episode \( k \). As the accuracy of the estimated model improves, the value of \( \epsilon_k \) increases.\yw{Do we still have dynamic \(\epsilon_{k}\)?}





% \yw{add justification in comments that Lipschitz assumption is reasonable.}


